The EDGE-CALIFA Survey: Spatially Resolved 13CO(1-0) Observations and Variations in 12CO(1-0)/13CO(1-0) in Nearby Galaxies on kpc Scales

We present 13CO(1-0) observations for the EDGE-CALIFA survey, which is a mapping survey of 126 nearby galaxies at a typical spatial resolution of 1.5 kpc. Using detected 12CO(1-0) emission as a prior, we detect 13CO(1-0) in 41 galaxies via integrated line flux over the entire galaxy, and in 30 galaxies via integrated line intensity in resolved synthesized beams. Incorporating our CO observations and optical IFU spectroscopy, we perform a systematic comparison between the line ratio R12/13 and the properties of the stars and ionized gas. Higher R12/13 values are found in interacting galaxies than in non-interacting galaxies. The global R12/13 slightly increases with infrared color F60/F100, but appears insensitive to other host galaxy properties such as morphology, stellar mass, or galaxy size. We also present annulus-averaged R12/13 profiles for our sample up to a galactocentric radius of 0.4r25 (~6 kpc), taking into account the 13CO(1-0) non-detections by spectral stacking. The radial profiles of R12/13 are quite flat across our sample. Within galactocentric distances of 0.2r25, azimuthally-averaged R12/13 increases with star formation rate. However, the Spearman rank correlation tests show the azimuthally-averaged R12/13 does not strongly correlate with any other gas or stellar properties in general, especially beyond 0.2r25 from the galaxy centers. Our findings suggest that in the complex environments in galaxy disks, R12/13 is not a sensitive tracer for ISM properties. Dynamical disturbances, like galaxy interactions or the presence of a bar, also have an overall impact on R12/13, which further complicate the interpretations of R12/13 variations.

==> center_stk_rs.tex <==
$I_{12}$ & & &
%$\log I_{12}$ (K km/s) & N_points & 52& N_gal & 32
 $0.50$ & $ < 0.001$ & & $0.27$ & $0.087$ & &$0.39$ & $0.22$ \\
$I_{13}$  & & &
%$\log I_{13}$ (K km/s) & N_points & 52& N_gal & 32
 $0.09$ & $0.55$ & & $-0.08$ & $0.62$ & &$0.06$ & $0.85$ \\
MOM2  & & & 
%MOM2 (km/s) & N_points & 52& N_gal & 32
 $0.13$ & $0.35$ & & $0.04$ & $0.81$ & &$-0.04$ & $0.91$ \\
$\Sigma_{*}$ & & & 
%$\log \Sigma_{*} (\mathrm{M_{\odot} pc^{-2}})$ & N_points & 52& N_gal & 32
 $0.15$ & $0.28$ & & $0.12$ & $0.46$ & &$0.45$ & $0.14$ \\
$Z_{mwt}$ & Mass weighted stellar metallicity& & 
%$Z_{mwt}$ ($Z_{\odot}$) & N_points & 52& N_gal & 32
 $-0.12$ & $0.38$ & & $0.06$ & $0.71$ & &$-0.45$ & $0.14$ \\
Age$_{mwt}$  & Mass weighted stellar age & & 
%$\log$ Age$_{mwt}$ (yr)  & N_points & 52& N_gal & 32
 $0.05$ & $0.73$ & & $0.02$ & $0.92$ & &$0.06$ & $0.85$ \\
Av & Extinction & & 
%$\log $Av & N_points & 52& N_gal & 32
 $0.24$ & $0.081$ & & $0.15$ & $0.36$ & &$0.21$ & $0.51$ \\
 12 + $\log$(O/H) & Gas phase metallicity & & 
 %12 + $\log$(O/H) & N_points & 45& N_gal & 28
 $0.16$ & $0.29$ & & $0.24$ & $0.16$ & &$0.52$ & $0.18$ \\
$\Sigma_{\mathrm{SFR}}$ & & & 
%$\log \Sigma_{SFR} (\mathrm{M_{\odot} yr^{-1} kpc^{-2})}$ & N_points & 45& N_gal & 28
 $0.43$ & $0.0035$ & & $0.45$ & $0.0055$ & &$0.17$ & $0.69$ \\
 $sSFR$ & & &
 %$\log \ $sSFR $(\mathrm{Gyr^{-1}})$ & N_points & 45& N_gal & 28
 $0.38$ & $0.0095$ & & $0.33$ & $0.043$ & &$0.52$ & $0.18$ \\
$\Sigma_{\mathrm{mol}}/\Sigma_{*}$ & & &
%$\log (\Sigma_{mol}/\Sigma_{*})$ & N_points & 52& N_gal & 32
 $0.58$ & $ < 0.001$ & & $0.31$ & $0.05$ & &$0.29$ & $0.35$ \\
$t_{\mathrm{dep}}$ & & & 
%$\log t_{\mathrm{dep}} (\mathrm{Gyr})$ & N_points & 45& N_gal & 28
 $-0.10$ & $0.52$ & & $-0.25$ & $0.14$ & &$-0.26$ & $0.53$ \\
